Riesz-type inequalities and maximum flux exchange flow

Let $D$ stand for the open unit disc in $\mathbb{R}^d$ ($d\geq 1$) and $(D,\,\mathscr{B},\,m)$ for the usual Lebesgue measure space on $D$. Let $\mathscr{H}$ stand for the real Hilbert space $L^2(D,\,m)$ with standard inner product $(\cdot,\,\cdot)$. The letter $G$ signifies the Green operator for the (non-negative) Dirichlet Laplacian $-\Delta$ in $\mathscr{H}$ and $\psi$ the torsion function $G\,\chi_D$. We pose the following problem. Determine the optimisers for the shape optimisation problem \[ \alpha_t:=\sup\Big\{(G\chi_A,\chi_A):\,A\subseteq D\text{is open and}(\psi,\chi_A)\leq t\,\Big\} \] where the parameter $t$ lies in the range $0<t<(\psi,1)$. We answer this question in the one-dimensional case $d=1$. We apply this to a problem connected to maximum flux exchange flow in a vertical duct. We also show existence of optimisers for a relaxed version of the above variational problem and derive some symmetry properties of the solutions.

==> DRAFT_6.tex <==
\section{The non-symmetric case, II}

\noindent In this case we take $t\in(0,\,1/3)$ and imagine a configuration that lies entirely in the right-hand interval $(0,\,1)$ but that has not yet been pushed rightwards to the maximum extent.  

\medskip

\begin{lemma}\label{lemma_on_non_symmetric_case_II}
Let $m\in\mathbb{N}$ and $t\in(0,\,1/3)$. Suppose that $f\in U^{(m)}_t$ satisfies the properties
\begin{itemize}
\item[{\it (i)}]
$(\,f,\,\chi_{(-1,\,0)}\,)=0$;
\item[{\it (ii)}]
$(\,f,\,\chi_{(0,\,\xi_t)}\,)>0$.
\end{itemize}
Then there exists $f_1\in U^{(m)}_t$ with the property that $f_1 = P\,f_1$ such that $J(f) < J(f_1)$.
\end{lemma}

\noindent{\em Proof.}
Again take $f=\chi_A$ where $A$ satisfies condition (\ref{condition_on_A}) and
suppose $f$ takes the form described at the beginning of the proof of Theorem \ref{optimality_criterion}. By {\it (i)}, $a_1\geq 0$ and by {\it (ii)}, $a_1<\xi_t$.
Therefore $a_1<b_1<1$; for otherwise, if $b_1=1$ then 
\[
(f,\,\psi) \geq (\chi_{(a_1,\,1)},\,\psi) > (\chi_{(\xi_t,\,1)},\,\psi) = t.
\]
Again borrowing the notation of Theorem \ref{optimality_criterion}, put
$f_1:=\chi_{A_1}$ and $f_2:=\sum_{j=2}^{k}\chi_{A_j}$. By Lemma \ref{evaluation_of_h},
\[
h_{f_1}(a_1)=\frac{1}{1-a_1}\int_{(a_1,\,b_1)}\big(\,1-x\,\big)\,dm = \frac{b_1 - a_1}{1-a_1}\left\{\,1 - (1/2)\big( a_1 + b_1 \big)\right\}
\]
and
\[
h_{f_1}(b_1)=\frac{1}{1+b_1}\int_{(a_1,\,b_1)}\big(\,1+x\,\big)\,dm = \frac{b_1 - a_1}{1+b_1}\left\{\,1 + (1/2)\big( a_1 + b_1 \big)\right\}.
\]
A little algebra yields $h_{f_1}(b_1) > h_{f_1}(a_1)$. Lemma \ref{evaluation_of_h} also indicates that $h_{f_2}$ is monotone increasing on $[-1,\,a_2]$. Therefore, $h(b_1) > h(a_1)$.
The conclusion now follows with the help of Theorem \ref{optimality_criterion}.
\qed

